Mixed-Criticality Scheduling with I/O

This paper addresses the problem of scheduling tasks with different criticality levels in the presence of I/O requests. In mixed-criticality scheduling, higher criticality tasks are given precedence over those of lower criticality when it is impossible to guarantee the schedulability of all tasks. While mixed-criticality scheduling has gained attention in recent years, most approaches typically assume a periodic task model. This assumption does not always hold in practice, especially for real-time and embedded systems that perform I/O. For example, many tasks block on I/O requests until devices signal their completion via interrupts; both the arrival of interrupts and the waking of blocked tasks can be aperiodic. In our prior work, we developed a scheduling technique in the Quest real-time operating system, which integrates the time-budgeted management of I/O operations with Sporadic Server scheduling of tasks. This paper extends our previous scheduling approach with support for mixed-criticality tasks and I/O requests on the same processing core. Results show the effective schedulability of different task sets in the presence of I/O requests is superior in our approach compared to traditional methods that manage I/O using techniques such as Sporadic Servers.

==> Makefile <==
PAPER = io_amc
TEX_FILES = $(PAPER).tex intro.tex abstract.tex related.tex conclusions.tex \
            ss_and_pibs.tex amc.tex amc_ss_and_pibs.tex experimental.tex    \
             implementation.tex blocking_io.tex
PDFV=okular
BIBLIO=io_amc.bib

all:
	$(MAKE) pdf

FIGURES=figures/*.eps

$(PAPER).dvi: $(TEX_FILES) $(BIBLIO) $(FIGURES)
	latex $(PAPER).tex
	bibtex $(PAPER)
	latex $(PAPER).tex
	latex $(PAPER).tex

dvi: $(PAPER).dvi

$(PAPER).ps: $(PAPER).dvi
	dvips -Ppdf -G0 -t letter -o $(PAPER).ps $(PAPER) # make better pdf w/ options

ps: (PAPER).ps

pdf: $(PAPER).pdf

$(PAPER).pdf: $(PAPER).ps
	ps2pdf  $(PAPER).ps


show: all
	$(PDFV) $(PAPER).pdf

black-white: all
	gs -sOutputFile=black-white.pdf -sDEVICE=pdfwrite \
	-sColorConversionStrategy=Gray \
	-dProcessColorModel=/DeviceGray \
	-dCompatibilityLevel=1.4 \
	-dNOPAUSE \
	-dBATCH \
	$(PAPER).pdf


clean:
	rm -rf *~ *.aux *.bbl *.blg $(PAPER).pdf $(PAPER).dvi *.log $(PAPER).ps
	rm -rf black-white.pdf

.PHONY: dvi pdf show clean all


==> blocking_io.tex <==
\textbf{This is a mistake in this analysis (off by 1 error) see textbf for more
info.  Remember there are two hard things in computer science: cache
invalidation, naming things, and off-by-one errors :-)}



The analysis presented in Sections~\ref{sect:ss_and_pibs}
and~\ref{sect:amc_ss_and_pibs} is designed to properly handle I/O events.  What
is missing from the analysis is the dependency between the main task and the I/O
event(s) the main task initiated.  Since the target domain for this analysis is
real-time and embedded systems we will assume main tasks are either purely CPU
bound or perform I/O using the following model for a job:

\begin{itemize}
\item The job performs some computation on an input, e.g. camera data
\item Optionally, the job performs a write I/O operation based on the said
  computation, e.g. sends actuator commands.  This write will not be blocking as
  the job will simply program the device and continue execution.
\item The job performs a read I/O operation for the next computation, this read
  is blocking in the sense that the task will require the data to perform the
  computation in the next job.
\end{itemize}

We assume the interrupts associated with the device have the following
properties:

\begin{itemize}
\item $K$ -- the number of bottom halves caused by the read I/O request
\item $B$ -- the time to process a single interrupt bottom half
\item $F$ -- the time between when the I/O request is initiated (i.e. the
  completion of the main task) and the first interrupt
\item $I$ -- the (maximum) inter-arrival time between interrupts
\end{itemize}
We assume $I{>}B$, otherwise the interrupts could be viewed as a single
interrupt as the suspension of the bottom half thread never needs to occur.

In order for an I/O job to start execution, the data requested at the end of the
last job must be available.  Therefore, the bottom half interrupt handlers must
be processed before the end of the main task's period.  To ensure that this
occurs an additional response time analysis test is required for the tasks that
handle bottom half threads.  For a system of only Sporadic Servers if $\tau_b$
that handles I/O bottom half handlers initiated by main task $\tau_i$ the
following is the response time analysis to ensure that $\tau_b$ will handle all
I/O bottom half threads before $\tau_i$ runs:

\begin{align}
  \label{eq:ss_blocking}
  R_b^{i} = R_i & + \left(B \times K\right) + F + \left(K - 1\right)\left(I -
  B\right) \notag \\ & + \sum_{j \in
    \mathbf{hp}\left(b\right)}\left\{\left(\left\lceil\frac{R_b^{i}}{T_j}
  \right\rceil - \left\lceil\frac{R_i}{T_j}\right\rceil \right)C_j\right\}
\end{align}

\textbf{I'm pretty sure we need to add 1 to the number of releases, this is
because a higher priority sporadic server could be waiting and comes in when
just when we need to execute.  This would be after the first iteration when the
Sporadc Server has for the interrupts has already executed and its replenishment
list is fragmented to align with the previous periods interrupt pattern.}

If $R_b^{i} {<} T_i$ then the interrupt bottom halves will be handled before the
main task starts execution again.  This is assuming $\tau_b$ has been assigned
sufficient capacity/utilization to handle interrupt bottom half threads.
Equation~\ref{eq:ss_blocking} is broken down into the following parts:

\begin{itemize}
  \item $R_i$ -- the worst case response time of task $\tau_i$.  It is also the
    worst case time the I/O read request will be initiated.
  \item $\left(B \times K\right)$ -- the time necessary to handle the interrupt
    bottom halves.
  \item $F + \left(K - 1\right)\left(I - B\right)$ -- the maximum time $\tau_b$
    will block due to waiting for interrupts.
  \item $\sum_{j \in
    \mathbf{hp}\left(b\right)}\left\{\left(\left\lceil\frac{R_b^{i}}{T_j}
    \right\rceil - \left\lceil\frac{R_i}{T_j}\right\rceil \right)C_j\right\}$ --
    the maximum interference experience from higher priority tasks during the
    handling of the interrupt bottom halves.  Specifically,
    $\left(\left\lceil\frac{R_b^{i}}{T_j} \right\rceil -
    \left\lceil\frac{R_i}{T_j}\right\rceil \right)$ represents the maximum
    number of releases of the higher priority task $\tau_j$ after $\tau_i$ has
    finished execution.  Execution of $\tau_j$ will interfere with $\tau_b$
    $C_j$ amount of time for each execution.
\end{itemize}

For a system of Sporadic Servers and PIBS Equation~\ref{eq:ss_blocking} can be
extended to include the interference caused by PIBS.  This added interference is
similar to the added interference caused by PIBS in Equation~\ref{eq:ss_rtb}.
\begin{align}
  \label{eq:ss_pibs_blocking}
  R_b^{i} = R_i & + \left(B \times K\right) + F + \left(K - 1\right)\left(I -
  B\right) \notag \\ & + \sum_{j \in
    \mathbf{hp}\left(b\right)}\left\{\left(\left\lceil\frac{R_b^{i}}{T_j}
  \right\rceil - \left\lceil\frac{R_i}{T_j}\right\rceil \right)C_j\right\}
  \notag \\ & +\sum_{\tau_k \in \mathbf{ps}}\max_{\tau_q \in
  \mathbf{hip}\left(i\right)}\left\{I_k^q\left(R_b^{i} - R_i\right)\right\}
\end{align}

Note that for the final term of Equation~\ref{eq:ss_pibs_blocking} the time
interval considered for the PIBS interference is $R_b^{i} - R_i$ as this is the
time window of interest for completing the interrupt bottom halves.

\subsection{Extending to Adaptive Mixed-Criticality}

The above formulation can be extended to Adaptive Mixed-Criticality.  The
interval model is extended to have both \HI{} and \LO{}-criticality interrupts,
similar to the \HI{} and \LO{}-criticality Sporadic Servers and PIBS.  We assume
the task assigned to handle the interrupt bottom half (either a Sporadic Server
or PIBS) is assigned the same criticality level as the bottom half threads.  The
previous interrupt model is extended by making $B$ a vector to represent the
time necessary to process a single interrupt bottom half in different
criticality modes.  Similar to traditional AMC, for a \LO{}-criticality
interrupt are defined by a $B\left(\mathtt{LO}\right)$ and do not run in
the \HI{}-criticality mode.  \HI{}-criticality interrupts are defined by both
$B\left(\mathtt{LO}\right)$ and $B\left(\mathtt{HI}\right)$ with
$B\left(\mathtt{HI}\right){>}B\left(\mathtt{LO}\right)$.

There will be three tests for ensure interrupts do not interfere with the
execution of the blocking main task.  The tests are for the \LO{}-criticality
steady state, the \HI{}-criticality steady state and the mode change
from \LO{}-criticality to \HI{}-criticality.  The two steady states are simple;
including all tasks using their \LO{}-criticality capacities/utilizations or
only the \HI{}-criticality tasks using only their \HI{}-criticality
capacities/utilizations.  The mode change is again the one of interest.

For a system of only Sporadic Servers the following is the response time
analysis:
\begin{align}
\label{eq:blocking_ss_amc}
R_b^{i*} = & R_i^{*}+ \left(B\left(\mathtt{HI}\right) \times K\right) + F + \left(K
  - 1\right)\left(I - B\left(\mathtt{HI}\right)\right) \notag \\
  &+ \sum_{\tau_j \in
\mathbf{hpH}\left(i\right)}{\left(\left\lceil\frac{R_b^{i*}}{T_j}\right\rceil -
\left\lceil\frac{R_i^{*}}{T_j}\right\rceil\right)
C_j\left(\mathtt{HI}\right)} \notag \\ &+ \sum_{\tau_j \in
\mathbf{hpL}\left(i\right)}{\left(\left\lceil\frac{R_b^{i*}}{T_j}\right\rceil -
\left\lceil\frac{R_i^\mathtt{LO}}{T_j}\right\rceil\right)
C_j\left(\mathtt{LO}\right)}
\end{align}

In Equation~\ref{eq:blocking_amc} the final two terms represent the additional
interference than can occur from high priority \HI{}-criticality
and \LO{}-criticality tasks, respectively, during the execution of the interrupt
handlers.

